Kernel Identification Through Transformers

Kernel selection plays a central role in determining the performance of Gaussian Process (GP) models, as the chosen kernel determines both the inductive biases and prior support of functions under the GP prior. This work addresses the challenge of constructing custom kernel functions for high-dimensional GP regression models. Drawing inspiration from recent progress in deep learning, we introduce a novel approach named KITT: Kernel Identification Through Transformers. KITT exploits a transformer-based architecture to generate kernel recommendations in under 0.1 seconds, which is several orders of magnitude faster than conventional kernel search algorithms. We train our model using synthetic data generated from priors over a vocabulary of known kernels. By exploiting the nature of the self-attention mechanism, KITT is able to process datasets with inputs of arbitrary dimension. We demonstrate that kernels chosen by KITT yield strong performance over a diverse collection of regression benchmarks.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> tables/uci_kernels.tex <==

\begin{table*}[t]
\centering

\begin{tabular}{l|l|l|c|c|c}
Dataset & $N$ & $d$ & Classification Transformer & Avg. RMSE & Avg. NLPD\\
\hline
Boston & 506 & 13 & MAT12, LIN*MAT52, LIN*MAT32 & 2.024 & 2.11 \\
Concrete & 1030 & 8 &   & \\
Energy & 768 & 8 &   & \\
Wine & 1599 & 11 &   & \\
Yacht & 308 & 6 &   & \\
Kin8mn & 8192 & 8 &  & \\
Naval &  11934 & 14 &  & \\
Power & 9568 & 4 & & \\
\end{tabular}
\label{ct_kernels}
\caption{Top 3 kernels predicted by the classification transformer across 10 splits.}
\end{table*}

